NoTeeline: Supporting Real-Time, Personalized Notetaking with LLM-Enhanced Micronotes

Taking notes quickly while effectively capturing key information can be challenging, especially when watching videos that present simultaneous visual and auditory streams. Manually taken notes often miss crucial details due to the fast-paced nature of the content, while automatically generated notes fail to incorporate user preferences and discourage active engagement with the content. To address this, we propose an interactive system, NoTeeline, for supporting real-time, personalized notetaking. Given micronotes, NoTeeline automatically expands them into full-fledged notes using a Large Language Model (LLM). The generated notes build on the content of micronotes by adding relevant details while maintaining consistency with the user's writing style. In a within-subjects study (n=12), we found that NoTeeline creates high-quality notes that capture the essence of participant micronotes with 93.2% factual correctness and accurately align with participant writing style (8.33% improvement). Using NoTeeline, participants could capture their desired notes with significantly reduced mental effort, writing 47.0% less text and completing their notes in 43.9% less time compared to a manual notetaking baseline. Our results suggest that NoTeeline enables users to integrate LLM assistance in a familiar notetaking workflow while ensuring consistency with their preferences - providing an example of how to address broader challenges in designing AI-assisted tools to augment human capabilities without compromising user autonomy and personalization.

==> Sections/NO-EDIT_Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
We describe the results of our user evaluation, both quantitatively and qualitative detailing the effectiveness of \tool. %The usage of each feature is reported in reference to system logs, recordings, ratings, and interviews. We also discuss the perceived limitations of the current prototype.

\subsection{\tool gives users more flexibility to take note}

\tool makes notetaking flexible because users need not write full notes anymore. We log how often users had to pause or rewind the video when taking notes (Figure \ref{fig:video_log}). Users paused or rewound less with \tool ( $ \mu =0.56, \sigma = 1.86$) compared to baseline ( $\mu = 4.94, \sigma = 5.97$).

%As users are not required to write fully furnished notes anymore in \tool, it gives users more flexibility. In Figure \ref{fig:video_log}, we report the log data on how many times users have to pause or skip the video while taking notes. We noticed that users tend to pause or seek backward/forward more frequently in baseline so that they can write the full note and do not miss any information. Whereas, in \tool, they did not pause and/or skip too much, since they have to write less now. Users paused and/or skipped in \tool less (mean=$0.56$, SD=$1.86$) than in baseline (mean=$4.94$, SD=$5.97$).

\begin{figure}
    \centering
    \hspace{-2pc}\includegraphics[width=0.8\linewidth]{images/video_log_dist.pdf}
    \caption{Distribution of pause and skips used by each participant in baseline and \tool.} %Participants paused more frequently in baseline compared to \tool.
    \label{fig:video_log}
\end{figure}

\textit{Users took shorter notes in \tool.}
%Users took shorter notes (i.e.: \textit{micronotes}) in \tool compared to baseline. 
We report the average length of notes written by users in \tool ( $\mu = 32.11, \sigma = 12.33$), shorter than that in baseline ( $\mu = 60.64, \sigma =16.94$) (Figure \ref{fig:image1}).

\textit{Users took more notes in \tool.} 
% We noticed that users tend to take more notes in \tool (Figure \ref{fig:image2}). 
The total number of notes is more in \tool ( $\mu = 18.75, \sigma =5.69$) compared to baseline ($\mu = 14.75, \sigma =2.59$) (Figure \ref{fig:image2}). 

\textit{Users took a shorter time to write notes in \tool.}
Compared to baseline ($\mu = 27.79, \sigma = 8.25$), the notetaking time was 43.9\% shorter in \tool ($\mu = 15.59, \sigma = 5.4$) (Figure \ref{fig:image3}). 

From the result, we can clearly see that \tool enables users to write more note points of shorter length in shorter time. It also reduces the video viewing distraction significantly. %As we will show in the following discussion, this significantly reduces effort in writing and users could focus more on the video content and understanding.

\begin{figure*}
\centering
\begin{subfigure}[b]{0.33\linewidth}
  \includegraphics[width=\textwidth]{images/len_note_points_dist_alt.pdf}
  \caption{Average length of note point.}
  \label{fig:image1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.33\linewidth}
  \includegraphics[width=\textwidth]{images/note_count_dist_alt.pdf}
  \caption{Total count of note point. %Most of the participants (except P2, P7, P10, P11) took higher amount of notes in \tool than in baseline.
  }
  \label{fig:image2}
\end{subfigure}
\hfill 
\begin{subfigure}[b]{0.33\linewidth}
  \includegraphics[width=\textwidth]{images/time_dist_alt.pdf}
  \caption{Average time per note point.}
  \label{fig:image3}
\end{subfigure}

\caption{Comparison of note length (a), count (b) , and writing time for each participant (c) between \tool and baseline. Majority of the users took higher amount of notes in \tool in less time.} 
\label{fig:threefigures}
\end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/len_note_points_dist_alt.pdf}
%     \caption{Average length of note point.}
%     \label{fig:image1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/note_count_dist_alt.pdf}
%   \caption{Total count of note point.}
%   \label{fig:image2}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/time_dist_alt.pdf}
%   \caption{Average time per note point.}
%   \label{fig:image3}
% \end{figure}

\begin{figure}
\centering
\begin{subfigure}[b]{0.3\linewidth}
  \includegraphics[width=0.9\textwidth]{images/tlx.pdf}
  \caption{}
  \label{fig:tlx}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\linewidth}
  \includegraphics[width=0.9\textwidth]{images/sus.pdf}
  \caption{}
  \label{fig:sus}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.3\linewidth}
  \includegraphics[width=0.97\textwidth]{images/time.pdf}
  \caption{}
  \label{fig:time}
\end{subfigure}
\caption{User study results (N=12). Boxplots from left to right: (a) workload measured with NASA TLX \cite{tlx} (7-point Likert
scale, lower is better), (b) usability measured with SUS \cite{sus} (7-point Likert scale, higher is better), (c) task completion time in seconds (lower is better).} 
\label{fig:ratings}
\end{figure}

\subsection{Analysis of \tool usage}

\subsubsection{Workload.} 
Using the Shapiro-Wilk test of normality, the differences between baseline and experimental condition responses for three of the four NASA-TLX questions \cite{tlx} on workload significantly deviate from a Normal distribution. Hence, we compare the differences in workload through a Wilcoxon One-tailed Signed-Rank Test \cite{neuhauser2011wilcoxon} with a Bonferroni-corrected \cite{weisstein2004bonferroni} significance level of 0.0125 per condition. Participants report significantly lower results for Mental Demand, Effort, and Frustration ($p = 0.0123, p= 0.0024, p = 0.0047$). We did not find statistically significance for higher Performance (p = 0.0803), this may be attributed to users feeling like they have not yet been able to make the best use of \tool, since they had just been introduced to the tool. For instance, P1 reflects on the UI could be "a little overwhelming" at first but that they "would get used to it." Further, likely due to users' general familiarity with notetaking, self-assessments of performance were already high in the baseline condition ($\mu = 5.58$ in the baseline vs $\mu = 6.25$ in the experimental condition on the 7-point Likert scale) and results may be subject to the ceiling effect (5 out of 12 participants gave the maximum 7 rating). %\todo{add some quotes}

\subsubsection{Usability.} 
Usability was measured via an adapted version of SUS \cite{sus}) and yielded an overall average of 80.972, which corresponds to an A grade according to the Sauro–Lewis curved grading scale \cite{sauro2016quantifying}. We note that the average baseline SUS values are also high at 80.833. Thus, our experimental features do not seem to detract from the inherent usability of notetaking methods more familiar to users. Further, our baseline condition already provides salient features that advance basic notetaking by 1) combining the video source and notetaking area into one video (five participants mentioned issues of screen space economy and the importance of a proper split screen setup during notetaking) and 2) providing an easily accessible summarizing feature—both of which received positive comments from participants (e.g. P12 mentions advantages of our setup over typical split screen set-ups for notetaking, which pose difficulties for tab navigation).
% I think it is ok if usability is not statistically significant - they are both quite high and usable

\subsubsection{Task Completion Time.} The differences in task completion times per participant across conditions pass the Shapiro-Wilk test of normality ($W = 0.8665, p= 0.0590$). Hence, we compare the differences in task completion times (seconds) through a parametric paired t-test. Participants report a significantly lower task completion time when using \tool ( $\mu = 207.7, \sigma = 17.25$) compared to the baseline ( $\mu = 322.36, \sigma = 103.27$) ($t(11)=3.6, p=0.004$)(Figure \ref{fig:time}).

. Um I felt like I had to like. Take every note you saw me like. pause and rewind at one point. point. Whereas in this. one and I felt like I could just watch it. all the way. through and not have to. to rewind.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/likert_scale_responses.pdf}
    \caption{Participants’ responses to utility and usability of \tool interface and various features (7-point Likert scale, higher is better).}
    \label{fig:enter-label}
\end{figure}

\subsubsection{Feedback on \tool features.} In figure \ref{fig:ratings}, we show participants rating for individual features in \tool ($\mu = 5.8, \sigma = 1.15$) (7-point Likert scale, higher is better). Overall, \tool was received positively by the users.

%\subsubsection{Usage patterns.}
%\textbf{Patterns of answering Cue Questions.} P1, .. referred back to their notes while doing the cue question testing. We also noticed participants preferred to keep their notes ordered by time rather than ordered by theme while answering the cue questions. However, this preference may change if more time passes between watching the video and attempting the cue questions.

%\textbf{Editing and reordering.} We noticed that some users reorganized the notes by dragging (P..).

\subsection{Discussion?/ Key Findings? / Themetic Analysis?}

\textbf{How do people create micronotes in \tool?:} Some example micronotes and their corresponding expanded notes created by our participants are reported in Table \ref{tab:example_notes}. Participants came up with different strategies while constructing their micronotes. We notice the use of symbols frequently. A commonly used symbol was '->' that denotes a process. We also noticed the use of '?' when the participants were unsure of the content or wanted to record a answer for a question. These symbols were accurately expanded via LLM in the final note. We also notice a high usage of abbreviation for certain words. For example, P1 used acronym, `\textit{BVI}' to represent `\textit{blind or visually impaired community}'. P2 used symbols `\textit{1}' and `\textit{2}' to represent two characters `\textit{Sam}' and `\textit{Felix}' from the video. Some participants used first one letter or a few following to write a word in short. For example, P8 wrote \textit{`l to r'} to mean \textit{`left to right'}.

%\textbf{Switch between micronote and expanded note.} Participants frequently jumped back and forth between the micronote and expanded note views. Some participants also liked to switch between them under the Theme view. P.. said `I apprecipate that it lets me see my original note, so that I can track what has changed into... Helps me recognize faster'.

\textbf{Do \tool features assist in notetaking? Why or why not?} \newline
\textbf{Reception of layout.} \todo{I might incorporate this section into something else since we didn't specifically ask about layout) Although several participants was accustomed to the side-by-side layout for notetaking in their usual tools,} three participants liked the top-to-bottom layout. P12 says: \textit{`I like the video + notes structure being upper/lower half, it makes sure that the two experiences are occurring at the same time.'} (users liked the timestamp signature for example, helps them know where it is linked back to find it easily.)

\textbf{Reception of expanded note.} All 12 participants reviewed some aspect of the expanded note favorably. All critical feedback, present in four of the responses, focused on the potential for verbosity and redundancy in the expanded notes. Still, nine reviews expressed appreciation for the quality/level of detail in the expanded note, and five reviews brought up that the expanded note captured details/context they would have otherwise missed.

% They liked the quality of the expanded note. p11: length seemed just right, not to short or long. follows the size of my note point. p7: it follows my writing style. I use a lot of '->' to represent a process in my note. P10: \textit{very detailed, concise, and grammatically correct}. however, some said the repetitive notes could be merged.

\textbf{Reception of generated themes.} Eleven out of 12 participants reviewed some aspect of the generated themes positively. Four reviews surfaced the possibility of content source/structure affecting the impact of the Order by Theme feature. P8 believes the impact of Order by Theme would become more evident in longer videos. P12 reflects on how "any video might have an introduction/conclusion with points that don't neatly fit into the content themes" and how the performance might vary across videos with "more narrative and structure... storytelling" that's time linear "rather than factual reasoning"—which also emerges in P1's response. P10 discusses how the Order by Theme feature would have greater impact in a video with more discursive content. In that regard, P11 expresses excitement about using the Order by Theme in such a context "where the conversation may not usually flow through on one topic." Five reviews specifically point out the utility of the Order by Theme feature for aiding review, retrieval, and organization of content.

% 'I like it. I think it is doing a better job than me.' 'Even if it is not perfect, it gives me an initial theme, os that I do not have to think too hard'.

\textbf{Reception of cue questions.} Eleven out of 12 participants reviewed some aspect of the cue questions positively, with critical feedback from five participants tending to focus on increased cue question complexity. Six participants specifically brought up positive impressions of the cue questions aiding in the video/note review process (e.g. ), four participants mentioned that they viewed the cue questions as a way to identify potential shortcomings in their notes, and three participants highlighted perceived relevance of cue questions to the video content.

% helps to revise, rather than testing? Some requested to have a difficult based cue question generation. It helps in the long run. P6: \textit{`I enjoyed being able to see the generated cue questions because it allowed me to review my notes and make sure that I had the most important points written down.. I think this would be extremely useful for reviewing lecture notes.'}

\textbf{Reception of summary.} Eleven out of 12 participants reviewed some aspect of the summary feature positively. Four responses brought up satisfaction with the summary's ability to capture the gist/important contexts from their notes. Three responses mentioned a preference for notes versus the generated summary for reviewing purposes: P1 prefers reviewing "small details" while P3 and P6 find the length too long. However, opinion on length is not uniform, as five responses (P5, P7, P8, P10, P12) reflected positively on the length of the summary. Four responses described a desire for more formatting features, such as bolded or highlighted text.

\textbf{Other emergent themes/incorporate into other sections... I'll take a look at my other list of themes tomorrow after full review}
\textbf{Incorporate into other sections}
-need for customization due to differences in preferences, matching writing style/what they "had in mind" 
-human-machine teaming


% People liked the personalized touch. P11 'It really tries to capture what I wanted'. Some preferred it to be a little less verbose. p10 'helpful for class notes, especially in high school, where I need to create a gist of summary of today's lecture'.

% \todo{Human-machine teaming}
% Time-saving
% AI - connections missed
% Feeling like a partner

% P1 - I am actively engaging in writing the smaller details down… And I would let the machine typically take over the higher level summary… That seems like a good division for me.
% P1 - useful cases in which I’ve missed a detail
% P3 - that’s a much better job than my notetaking
% P4 - details wasn’t able to manually catch
% P6 - I think there are some themes that I wouldn’t even have come up with.
% P9 - helpful context

% \textbf{Dragging and Editing}. compared with notion

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Micronote} & \textbf{Expanded note} \\ \midrule
RNNs are unrolled \colorbox{table_color_1}{l to r or opp} & Recurrent neural networks (RNNs) can be unrolled either from \colorbox{table_color_1}{left to right or from right to left}, encoding \colorbox{table_color_4}{linear locality}. \vspace{8pt} \\
find the average / adding vectors together & Average of vectors \colorbox{table_color_2}{-\textgreater} add vectors together \colorbox{table_color_2}{-\textgreater} find mean value. \vspace{8pt}\\
red \colorbox{table_color_5}{-\textgreater} all similar reds & Red color categorization \colorbox{table_color_5}{includes} various shades that are perceived as similar. \vspace{8pt}\\
Cites difficulties for \colorbox{table_color_1}{BVI} people & \begin{tabular}[c]{@{}l@{}}The speaker cites the difficulties faced by \colorbox{table_color_1}{blind and visually impaired} individuals, such as the \colorbox{table_color_4}{inability to independently} \\ \colorbox{table_color_4}{read books, magazines, or use computers and smartphones} without assistance.\end{tabular} \vspace{8pt}\\
sauce: \colorbox{table_color_3}{gehra?} & \begin{tabular}[c]{@{}l@{}}The sauce, known as \colorbox{table_color_3}{garum}, was a \colorbox{table_color_4}{staple in Ancient Greek and Roman cuisine}, valued for its strong umami flavor and \\ produced in large quantities throughout the Mediterranean.\end{tabular} \vspace{8pt}\\
\colorbox{table_color_1}{both} rich and umami & \colorbox{table_color_1}{Tomatoes, like fish sauce}, are rich in \colorbox{table_color_4}{glutamate} which gives them a strong umami flavor. \vspace{8pt}\\
css property \colorbox{table_color_5}{--\textgreater} native styling & Custom properties in CSS can be used to \colorbox{table_color_5}{create} native styling options for web design. \vspace{8pt}\\
\colorbox{table_color_1}{met} & The \colorbox{table_color_1}{Metropolitan Museum of Art} is located on Fifth Avenue and spans five blocks. \vspace{8pt}\\
))) \colorbox{table_color_5}{-} russian & In Russian, multiple closing brackets ")))" \colorbox{table_color_5}{indicate} \colorbox{table_color_4}{varying degrees of happiness} in a smiley face. \vspace{8pt}\\
pipe \colorbox{table_color_5}{--\textgreater} high to low pressure & Water in pipes \colorbox{table_color_5}{flows from} areas of high pressure to low pressure, similar to how electrons move from high to low voltage. \vspace{8pt}\\
equipment durability & \colorbox{table_color_4}{Cycling pumps} on and off to meet variable demand increases wear and tear, affecting equipment durability. \vspace{8pt}\\
slow - reducing fat mass. fast \colorbox{table_color_5}{-} reducing \colorbox{table_color_3}{muscule} mass & Slow dieting reduces fat mass, while fast dieting \colorbox{table_color_5}{leads to} \colorbox{table_color_3}{muscle} mass loss. \vspace{8pt}\\
\colorbox{table_color_1}{1} \colorbox{table_color_3}{enery} deficit & \colorbox{table_color_1}{Sam} creates an \colorbox{table_color_3}{energy} deficit by \colorbox{table_color_4}{consuming fewer calories and increasing exercise}, leading his body to break down glucose stores. \vspace{8pt}\\
loose fast\colorbox{table_color_5}{? \textless} find healthier life style & Losing weight quickly isn't ideal; \colorbox{table_color_5}{instead}, focus on discovering a lifestyle that promotes personal health and happiness. \\ \midrule
\multicolumn{2}{c}{\textbf{Applied Changes:} \colorbox{table_color_2}{\vphantom{X}\hspace{0.8em}} Mimic Personal Writing Style\vphantom{X}\hspace{1.5em}  \colorbox{table_color_1}{\vphantom{X}\hspace{0.8em}}  Abbreviation Expansion \vphantom{X}\hspace{1.5em}\colorbox{table_color_3}{\vphantom{X}\hspace{0.8em}} Fix Typo\vphantom{X}\hspace{1.5em}  \colorbox{table_color_4}{\vphantom{X}\hspace{0.8em}}  Extracted Detailed Information\vphantom{X}\hspace{1.5em} \colorbox{table_color_5}{\vphantom{X}\hspace{0.8em}}  Personalized Symbolic Interpretation} \\ \bottomrule
\end{tabular}%
}
\caption{Example micronotes and the expanded notes created by our participants during the user study. The relevant portions in the micronote and expanded note have been highlighted for readability.}
\label{tab:example_notes}
\end{table*}

\begin{mdframed}[style=MyFrame]
\faIcon{hashtag} \textbf{Takeaway:}  2. The system should have atomic level customization at each step of the process.
- hierarchical information viewing
- atomic / granular customization (one participant said they would like to customize the layout and menu color. One said they would like the summary style in their control. Tldr: give them agency and control, however, show them gradually so that they are not overwhelmed) 

3. if LLM is used, really show the reference to show it is not hallucinating

(users liked the timestamp signature for example)

4. how to design an interface in privacy preserving way without requiring a lot of data for personalization

4. if LLM is used, properly notify the errors to users. 
\end{mdframed}

\subsection{How people envision using \tool}
During the freeform test (\textsection \ref{subsec:vid_select}), Participants reported a wide range of use cases where \tool can be useful in their daily lives. All 12 participants wished to continue using \tool in future. P7 continued using \tool for annotating interviews collected as part of their research even after our study session. P9 mentions the desire for integration with a current Learning Management System, Canvas, used at their university. Most participants thought \tool is useful for long-form videos where there is a lot of information to capture rather than short videos which may not that essential to take notes on. The top categories they reported are: 1. \textit{Educational Video Content ($\times8$)} 2. \textit{Professional Podcast and meetings ($\times3$)} 3. \textit{Thematic analysis of research videos ($\times3$)} 4. \textit{Personal Learning and Self-Education from how-to tutorials ($\times2$)} 5. \textit{Financial and Investment Learning ($\times1$)}. 

%P11 commented that he watches a lot of interviews and podcasts and wants to remember certain quotes by the speakers that \tool can help with. P7, .. thought it would be useful for coding tutorials. 

Even when features were not immediately relevant to their current needs, some reported potential uses for others or themselves at other time points in their lives. P12 says the cue questions would be useful for \textit{`my (their) friends at med school'}  where `\textit{the details get really granular and... the names of things can can make or break like the answer to a question.'} P6 mentions how, even though they are no longer a student, they would have `\textit{definitely want[ed] to use [\tool] with [their] lectures... freshman and sophomore year when classes were online.'}

Two participants thought \tool is not be applicable to leisure viewing such as \textit{`TV shows or movies with friends since I'm not taking notes in those cases (P4).'} P9 thought it may not be applicable to philosophical contents such as \textit{`humanities where concepts are more open to interpretation'}, rather than a factual information.
\newline
\begin{mdframed}[style=MyFrame]
\faIcon{hashtag} \textbf{Takeaway:}  notetaking needs for different video domains is different. Hence, features of notetaking tool must be specific to target video domain and duration. Similar trend is also found in video editing tools \cite{mannessh1, maneesh2, maneesh3}.  
\end{mdframed}

% \subsection{Design Implication}
% what we learned from noteeline that can be helpful for building better notetaking tools as a guideline which are beyond generic human-ai guidleines and is more specific to notetaking tool

% bnous point: refer back to our design rationale. not exact repetiion, maybe combining them as well

% what we already is good, that can be also be included and implemented in future works, rather than the limitation (which is mentioned in the future work section)




==> Sections/demo_main_body.tex <==
\section{Introduction}
\vspace{5pt}
\begin{quote}
% https://www.goodreads.com/quotes/9537930-the-more-content-you-try-to-capture-during-a-lecture
    \textit{"The more content you try to capture during a lecture or a meeting, the less you're thinking about what's being said. You burn through most of your attention parroting the source." - Ryder Carroll \cite{carroll2018bullet}} \\ 
\end{quote}


% \todo{1st para - why it is helpful to write micronote}
With the rise of platforms like Youtube, TedEx, Khan Academy; video has emerged as a popular form of communication and information sharing \cite{tversky2002animation, betrancourt2018and}. %Though video platforms have made videos more accessible, users still face challenges capturing notes from videos. 
These platforms have made accessing videos easier than ever. However, users often face significant challenges when it comes to capturing notes from these videos \cite{shoufan2019estimating, tabbers2004multimedia, Boyle2007ThePO}. The main difficulty lies in the cognitive load required to take comprehensive notes while simultaneously processing and understanding new information \cite{Piolat2005CognitiveED, JANSEN2017223, workingmemperf}. This cognitive load can demotivate users, leading to lower-quality notes or even causing them to forego note-taking altogether \cite{Kafipour2021ProcrastinationAI, flanigan2020impact, mccoy2020gen, bui2013note}. % As a result, despite the accessibility of video content, the challenge of effective note-taking remains a barrier for many users.

Previous research on active note-taking tools has explored various methods to assist users in taking notes more efficiently \cite{subramonyam2020textsketch, Chiu1999NoteLookTN, VideoSticker}. While these notetaking tools provide user-friendly features for describing and categorizing notes faster, users still need to manually write the full notes, one of the primary factors that make notetaking challenging \cite{Piolat2005CognitiveED}. With advancements in language processing and Large Language Models (LLMs), recent tools have been using LLMs to generate notes or summaries from videos and live lectures \cite{notegpt_2024, Notion, otter}. However, these notes are generated \textit{automatically} without any user involvement. As a result, they are often not \textit{personalized} to the users' preferences \cite{biermann2022tool}. % notetaking objectives. 

% - We would like users instead to take MICRONOTES
% - However, the challenge with only writing micronotes, it they are not useable later
% - So we build an expansion tool that support micro-notetaking

In this work, we %propose letting users take \textit{micronotes} \cite{micronote}. 
aim to bridge these gaps by enabling users to take less demanding \textit{micronotes} \cite{micronote} and then \textit{automatically} expanding them into full-fledged notes. By \textit{micronote}, we refer to scribbles composed of \textit{couple-of-words} and informal notations \cite{micronote, shorthand_tt}. These micronotes are concise, causing minimal viewing distraction while capturing essential information densely. We developed a proof-of-concept interface, \textit{NoTeeline} (Figure \ref{fig:teaser}) that allows users to write such micronotes and utilizes the relevant context in the video to create the full \textit{(expanded)} note. Micronotes being extremely brief, we need additional context to expand them properly \cite{Monty1986TEMPORALCA}. \textit{NoTeeline} efficiently achieves this by utilizing the video transcript and previous examples of user micronotes in reference videos.% to decode the micronotes properly. 

\section{\tool Interface}

\begin{figure*}
    \centering\includegraphics[width=0.7\linewidth]{images/ui.pdf}
    \caption{The \tool user interface consists of (a) the \textit{Cues} panel (outlined in blue) for review questions generated based on the notes, (b) the \textit{Notes} panel (outlined in orange) for user notetaking and note expansion, and (c) the \textit{Summary} panel (outlined in purple) for note summary. The layout is inspired by the Cornell method, as seen in the side-by-side comparison.}
    \label{fig:ui}
\end{figure*}

\subsection{Design Goals}
% Rambler is built around the creation and manipulation of Rambles, illustrated in Figure 1 and 2. Each Ramble is a container (visually separated from other Rambles) that holds its content and multiple buttons for users to interact with. Our intention is for the content of a Ramble to roughly correspond to a single train of thought. Without the pressure of producing a decent piece of text in one shot, users may either speak everything into one Ramble and split it later, or start a new Ramble when they feel what they will say next is about a different point or subject matter. Rambler should support various writing strategies, including those starting both with or without an outline in mind. Here, we explain the design of Rambler and its main features supporting macro revision and text reviewing, respectively

% Based on fndings from the formative study and the iterative prototyping and evaluation process, we derive four design goals for a diagram-oriented interaction with LLMs. We frst describe the Design goals, and then a scenario (Section 5) to ground how these goals can be supported by a novel system and lead to fuid interaction with LLM-generated information

% Core to our system is the concept of \textit{micronote} \cite{micronote, shorthand_tt}. 
% We propose three design goals for \tool.

D1. \textit{Micronotetaking as the way to take notes from videos.} The interface should enable the swift creation of micronote. Even if the micronote includes grammatical errors and/or is extremely small as 1 word, the system should be able to process it. While transforming micronotes, it should be aware of the context, i.e: the topic being discussed in the video. The system should enable iterative editing of micronotes. %By focusing on micronotes, we want to tackle the difficulty in writing full notes users mentioned in C1.

D2. \textit{Maintain consistency with user's style and preferences.} The system should take into account the specific writing styles each user follows and remain consistent with their personal style. At the same time, the final note should exclude information users are not interested in. %It should not include any hallucinated information, as desired by the participants in our findings, C2.

D3. \textit{Each component is linked to a specific note-taking procedure and shown accordingly.} The system should link each component to a specific stage in the note-taking process — creation, editing, and revision. It should allow users to engage selectively with these features based on the current stage, providing ease of use throughout the note-taking journey \cite{pea1987user, nielsen_2006}. %, so that it does not overwhelm the users mentioned in C3. %Each individual component is linked with a specific note-taking stage: note creation, editing and revision. The system should allow users to selectively engage with different features at their will as per their need \cite{pea1987user, nielsen_2006}. %The disclosure of these features should follow the flow of standard notetaking practices 
% https://en.wikipedia.org/wiki/Progressive_disclosure 

% \textit{D3. Ensure contextualized creation of note.} While expanding and transforming micronotes, the interface should be aware of the context, i.e: the topic being discussed in the video. At the same time, the final note should exclude information users are not interested in. It should not include any hallucinated information.

%\textit{D3. Maintain consistency with personal writing style.} The system should take into account the specific writing styles each user follows and remain consistent with their personal style.

%\textit{D4. Assist in iterative editing and review.} The interface should enable users to edit and review any automatically generated text.

%\textit{D5. Leverage automation while preserving user control.} The interface may leverage the benefits of automation, but it must ensure that users maintain authority over the extent of modifications.

% \textbf{D1. Conditional expansion/creation of note}: Existing AI based notetaking tool utilizes the audio transcript to generate keypoints. These keypoints are generated automatically and are not controllable by the user. Compared to these tools, our notetaking tool will enable the users to set the initial keypoints for notes to expand on them. By doing so, we build a user-in-the-loop interaction that gives them automated notes while having control over it.

\subsection{Interface Components}

We will now describe the components of \tool built to support our design goals.

% \begin{figure}
%     \centering\includegraphics[width=0.9\linewidth]{images/onboarding.jpg}
%     \caption{During the onboarding session, the user would write both  short keypoints and a full note for several short video clips.}
%     \label{fig:onboarding}
% \end{figure}

\subsubsection{\textbf{Onboarding Session: Collecting Personalized Examples.}} We design an onboarding session to get reference examples of the user's specific style (D2). Users watch three short clips (20-30 seconds each); and provide a keypoint as well as the corresponding full note for each clip (Figure \ref{fig:ui}). Once completed, the system will store these examples to use for note expansion afterwards. 

\subsubsection{\textbf{Notetaking Layout}.} To construct the layout, we took inspiration from the Cornell method  \cite{pauk2010study}, a popular technique for taking note \cite{Saran2022AnIT, workingmemperf}. %Cornell notes focuses on taking, organizing, and summarizing notes for better overall comprehension \cite{Saran2022AnIT, workingmemperf}.
We split \tool layout into three regions -- 1) \textit{\textbf{Notes}}: the region for writing and organizing note; 2) \textit{\textbf{Cues}}: questions or specific points that are helpful to review the note; and 3) \textit{\textbf{Summary}}: main takeaway of the note in 5 sentences. %We also incorporated the video viewport on the top of the layout so that users can take notes as they watch the video without needing the move between different desktop tabs (C4). It also progressively discloses the features as the users advance in their notetaking activities (D3). %\todo{We purposefully adopted a top-to-bottom layout rather than a side-by-side layout to allow users to have more space for text and a larger video viewing region.} 
Figure \ref{fig:ui} illustrates the notetaking layout and its different components. 

\subsubsection{\textbf{Note Synthesis Operations.}} \label{subsec:synthesis}
We describe individual synthesis operations \tool supports and their mechanism. \newline
\textbf{\textit{Micro Note Expansion.}} To construct the full note, we have an atomic \textit{expansion} operation. For \textit{expansion}, we utilize these pieces of information in the prompt: micronote, video transcript where the micronote was written, and reference examples from onboarding. %We empirically decided to take the transcript within a 20 seconds window when the micronote was created. 
The transcript helps to infer abbreviated symbols and fix potential typographical error (D1) \cite{context_helps}. Reference examples helps to understand users' writing style (D2).

\textbf{\textit{Note Organization by Theme.}} To rearrange the note points by emerging themes, we have an atomic \textit{order by theme} operation (D1, D3). To \textit{order by theme}, we pass the generated notes to the LLM and instruct it to return the output in a structured, parseable format by using the few-shot prompting technique \cite{Graphologue, openai_2023}.

\textbf{\textit{Note Modification.}} To edit individual micronote or the expanded output from LLM and/or the automatically generated theme name (D3), users can click on the \includegraphics[height=0.8em]{images/edit_note.png} button next to each point.

\textbf{\textit{Note Rearrangement.}} Users can drag individual note points and reposition them under a different theme using this operation. Users can also revert the note to its original serial by \textit{order by time} operation.
% To revert the note into its original serial, user have to perform the \textit{order by time} operation by clicking \includegraphics[height=0.8em]{images/order_time.png} button.

\textbf{\textit{Cue Question Generation.}} To enable users review their notes, we have a \textit{Cue Question Generation} operation, which generates 5 questions on-the-fly. If users want new questions, they have the option to initiate \textit{Regeneration} operation, which generates five new questions. The cue column is hidden by default to provide more space for writing to the users (D3).

% They can easily toggle between the cue and note layout using the \includegraphics[height=0.8em]{images/toggle_2.png},\includegraphics[height=0.8em]{images/toggle_1.png} buttons. 

\textbf{\textit{Summary Generation.}} To generate a personalized summary, we have a \textit{Summarize} operation. The generated summary needs to reflect the user's note as well as the video context (D2). Hence, we passed the full video transcript and expanded note to LLM for the summary. %We first preprocess the transcript into chunks using LangChain Map Reduce pipeline \cite{dean2008mapreduce, LangChain} before creating the final summary so that it does not exceed the input length of the LLM. 
% By pressing \includegraphics[height=0.8em]{images/summary.png}, users will be able to see the personalized summary created on their note in the bottom of the page. 

% 2. Video region (Video viewing): paste a url and press \includegraphics[height=0.8em]{images/submit_yt.png}

\subsection{System Walkthrough}

We present a hypothetical scenario to illustrate how users might interact with \tool. Kate is preparing a presentation on `\textit{Ocean Pollution}.' She uses \tool to watch a long 40-minute and gather information faster. She starts by completing the onboarding session and opens a new note named `\textit{Ocean Pollution Presentation}.' As she starts watching the video, Kate encounters a segment explaining the drastic increase in plastic pollution over the last decade. She quickly types "\textit{plastic pol. $\rightarrow$}" as a micronote. Once the video concludes, she presses the \includegraphics[height=0.8em]{images/expand.png} button, and \tool elaborates her micronote into a detailed point, including the specific statistic: "\textit{Plastic pollution in \textit{oceans} has increased by 200\% in the last 10 years.}" This expansion allows Kate to easily integrate precise details into her presentation later. 

Now, Kate needs to organize her thoughts into themes so that she can design the slide decks accordingly. To achieve this, Kate experiments with the \includegraphics[height=0.8em]{images/order_theme.png} feature. \tool organizes her notes into three themes - `\textit{Causes of Ocean Pollution}', `\textit{Effects on Marine Life}', and `\textit{Conservation Efforts}'. While she is happy with the themes, Kate decides to further personalize the themes. She notices a point 'biodegradable alternatives to plastic' that would be better suited under `\textit{Conservation Efforts}'. Kate drags it under it and renames the theme to `\textit{Sustainable Solutions}' to better align with her presentation structure.

Feeling content with the organization of her notes, Kate clicks on \includegraphics[height=0.8em]{images/summary.png} to generate a personalized \textit{TL;DR} summary of her insights for her conclusion slide.

Finally, Kate wants to anticipate potential questions from her audience. She opens the \includegraphics[height=0.8em]{images/cue_question.png} panel. 
% \tool shows five questions to her, including one on the most effective conservation efforts identified in recent studies.
Attempting to answer from memory, Kate correctly addresses the first question but stumbles on the second, prompting her to revisit her notes for a quick recap. %refresher on the specific points discussed. 
Satisfied with her understanding and the comprehensive coverage of her topic, she confidently moves on to finalizing her presentation, equipped with a well-structured and informative slide deck.


% Kate -- a rising junior -- is making a class presentation for her final class on 'Plastic Waste and its affect'. but the video is too long, so she wants to use \tool to capture micro note and focus more on the concent. \tool expands them into ... with the statistics details so that she can quickly copy paste it later on. order by theme helps her to organize the slide deck of her class. summary to create a suitable conclusion for her slide. Finally, cue question to understand what kind of questions peopple can ask her in the presentation.

% completes the onboarding session. loads the video -> starts watching video -> whenever she wants to note something, she writes it a keyowrd (give an example here). once she is done with waitching the video, she presses expand and reviews the note. She edits a note point '...'. Then, she tries out the 'order by theme' ..., which orgnaizes the points into the themes. she did not like one point (...), so she drags it under '..' theme and rename the theme to '..' to reflect the changes. Once she is happy with her note, she clicks 'summary' to get q personalized tldr of her note, so that she can revisit it later. in the last, she opens the cue question panel and clicks '..' to generate multi-choices questions. she ties to answer them from her memory. she gets the first one correct, for the third one ..... so, she quckly goes back to the note and revisits the concept again. Once she is happy with the full note and her leanring objective, she moves on to the next topic.  

% make it more technical, not specifically mention treadmill. 
% look into ramblers and dataparticle to write the case study

\section{Conclusion and Future work}
Although videos are a popular source of information seeking, notetaking from videos remains challenging. While existing tools can automatically generate notes, they can not capture the stylistic nuances users care about. An automatically generated summary may not be always accurate and/or customized properly. On the other hand, \tool leverages rich contextual information to generate more accurate and more personalized notes. \tool addresses these two issues by allowing users to use micronotes which are easier to write and can be automatically expanded with high accuracy. In future, we would like to extend \tool to support non-textual note taking (i.e: sketching and screenshot attachment). We also plan to formally evaluate \tool in user studies to understand what behaviors can emerge from more flexible note taking system.
% Our user study reveals that \tool helps write notes faster with $93.2\%$ correctness and achieves closer stylistic characteristics to users' handwritten notes. We demonstrate the utility of \tool in a variety of usage scenarios users reported.

==> Sections/technical_eval.tex <==
\section{Technical Evaluation}
\label{sec:tech_eval}
In this section, we quantitatively evaluate the constructed notes in \tool. 

\subsection{Consistency with Personal Writing style}
To understand if the generated notes in \tool mirror the nuances of a user's personal writing style, we conduct a stylometric analysis \cite{stein2007intrinsic, li2023automatic, argamon2010structure} using Mendenhall’s composition characteristic curve \cite{mendenhall1887characteristic} and Kilgariff’s Chi-Squared \cite{kilgarriff2001comparing} methods.
These methods compare the choice of words and their distribution to infer the writing style. The closer the distribution curves are, the higher their style similarity. In Figure \ref{fig:mcurve}, we can see that the word distribution of notes closely aligns with P11's hand-written note\footnote{For space limitation, we randomly show the curve of one participant. The rest exhibit the similar trend. More details can be found in our supplementary material.}, when we utilize the onboarding examples during note generation. The Chi-squared distance to the handwritten note is $224.38$ and $294.64$, respectively with and without using onboarding (lower is better). The results indicate that \tool achieves a better style match using the provided onboarding examples \cite{ning2024userllm}.

% - Saying something on the closer the curves are together, means higher writing similarity.
% - When we remove onboarding, the curves differ a lot, suggesting the importance of the onboarding session in helping expansion notes be similar to the writing style.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/mcurve_p11.pdf}
    \caption{Composition Characteristic curve for P11. The onboarding session examples help \tool generate notes in a similar style that user would write themselves (a closer curve indicates higher stylistic similarity.)}
    \label{fig:mcurve}
\end{figure}

\subsection{Note quality of \tool}
\textbf{\textit{Linguistic Property.}} We report the linguistic quality (in terms of \textit{grammaticality, non-redundancy, focus}) of notes using GRUEN~\cite{zhu2020gruen}. The result (Table \ref{tab:gruen_scores} in Appendix) indicates that the points written using \tool ($ \mu = 0.84, \sigma = 0.07$) are of higher quality (i.e: less grammatical less, less redundant and more focused) than the baseline ( $\mu = 0.56, \sigma = 0.17$) ($p < 0.0001, t(11)=10.87$).

\textbf{\textit{Correctness}.} To ensure our automatically expanded notes are indeed correctly extracting the information from the transcript and not hallucinating any misinformation, we compute the factual correctness of the generated note using HHEM \cite{vectara2024, zhang2023language, azamfirei2023large}. We noticed a Hallucination Rate = $4.97\%$ and a Factual Consistency Rate = $95.03\%$. This indicates that our generated notes are correct and consistent $95.03\%$ times. 

\subsection{Consistency of summary and note}
\label{subsec:cons_sm}
To measure if the generated summary is indeed personal and focuses on the points mentioned in the note, we measure the widely used sentence representation similarity using SBERT between the note and generated summary\cite{sbert, ethayarajh2019contextual, gao2019representation}. Compared to the baseline, \tool summary is 11\% more relevant to the user note (Table \ref{tab:relevance}). %We also provide an example in Figure ? from P11 where he watched a 40-minute-long video, but only took notes in the first 9 minutes. As desired, the generated summary mostly focused on the content spoken within the first 9 minutes rather than the following 31 minutes.


\begin{table}[]
\resizebox{\linewidth}{!}{%
\begin{tabular}{llllllllllllll}
 & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P6} & \textbf{P7} & \textbf{P8} & \textbf{P9} & \textbf{P10} & \textbf{P11} & \textbf{P12} & \textbf{avg.} \\ \hline
 \multicolumn{14}{c}{\textit{Consistency of Summary \& Note in two conditions (\textsection \ref{subsec:cons_sm})}} \\ \hline \\
Baseline & 0.81 & \textbf{0.53} & 0.81 & 0.61 & 0.64 & 0.76 & 0.33 & 0.67 & 0.65 & \textbf{0.71} & 0.44 & 0.72 & 0.64 \\
NoTeeline & \textbf{0.87} & 0.51 & \textbf{0.9} & \textbf{0.63} & \textbf{0.91} & \textbf{0.77} & \textbf{0.67} & \textbf{0.8} & \textbf{0.68} & 0.7 & \textbf{0.76} & \textbf{0.82} & \textbf{0.75} %({\color[HTML]{009901} \textbf{+11\%}})
\\ \\ \hline
\multicolumn{14}{c}{\textit{Consistency of Micronote, transcript \& corresponding expanded note (\textsection \ref{subsec:cons_mf})}} \\ \hline \\
\begin{tabular}[c]{@{}l@{}}Micronote \& \\ Expanded Note\end{tabular} & 0.6 & 0.41 & 0.73 & 0.75 & 0.63 & 0.58 & 0.55 & 0.6 & 0.48 & 0.43 & 0.57 & 0.63 & 0.58 \\ \\
\begin{tabular}[c]{@{}l@{}}Transcript \& \\ Expanded Note\end{tabular} & 0.47 & 0.41 & 0.42 & 0.42 & 0.42 & 0.39 & 0.42 & 0.42 & 0.44 & 0.46 & 0.39 & 0.41 & 0.42 \\ \hline 
\end{tabular}%
}
\caption{Technical Evaluation Result (measured as \textit{sentence representation similarity} \cite{sbert}, higher is better)}
\label{tab:relevance}
\end{table}

\subsection{Consistency of micro note and its corresponding expanded note}
\label{subsec:cons_mf}
% We measure the semantic similarity (BertScore) \cite{sbert} between micronote and expanded note to test if they are consistent with each other. We find that they have a 58\% similarity. %This indicates that while expanded notes stay true to the core ideas of the micronotes, they also include detailed information not mentioned in the micro note. These details are extracted from the provided transcript. 
% To ensure these expansions don't merely replicate the video's transcript (D2), we also examine the similarity of the expanded note and the transcript. We found it to be only 42\%. This low overlap confirms that our expanded notes prioritize the micronotes' content, carefully adding details from the video without changing the main message.

We measure the sentence representation similarity (using SBERT) \cite{sbert, ethayarajh2019contextual, gao2019representation} between micronote and expanded note to test if they are consistent with each other. We find that they have a 58\% similarity (avg. score = 0.58). We also examined the similarity of the expanded note and the transcript and found it to be 42\% (avg. score = 0.42). The expanded notes are more similar to micronotes than the transcript, indicating that our expanded notes prioritize the micronotes' contents and do not merely replicate the video transcripts.

% \begin{table}[]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llllllllllllll}
%  & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P6} & \textbf{P7} & \textbf{P8} & \textbf{P9} & \textbf{P10} & \textbf{P11} & \textbf{P12} & \textbf{avg.} \\ \hline 
% \begin{tabular}[c]{@{}l@{}}Micronote \& \\ Expanded Note\end{tabular} & 0.6 & 0.41 & 0.73 & 0.75 & 0.63 & 0.58 & 0.55 & 0.6 & 0.48 & 0.43 & 0.57 & 0.63 & 0.58 \\ \\
% \begin{tabular}[c]{@{}l@{}}Transcript \& \\ Expanded Note\end{tabular} & 0.47 & 0.41 & 0.42 & 0.42 & 0.42 & 0.39 & 0.42 & 0.42 & 0.44 & 0.46 & 0.39 & 0.41 & 0.42 \\ \hline 
% \end{tabular}%
% }
% \caption{Semantic similarity (measured as \textit{BertScore} \cite{sbert}, higher is better) of micro note, its corresponding expanded note and provided transcript in \tool. \tool successfully expands the micro notes into full notes while preserving the semantic meaning and not being an exact copy of the transcript.}
% \label{tab:relevance}
% \end{table}

\subsection{Error Analysis}
\subsubsection{Repetitive Pattern induced by temporal proximity.} 
\label{subsec:rep}
%We noticed that if the interval between two note points is minimal (i.e.: below 10 seconds), the content of the expanded notes tends to exhibit a high degree of similarity. For example, in scenarios where two points are written within less than a 10-second gap, the resultant average cosine similarity among them is  0.63. The reason for this error might be due to the amount of overlapping information present in both points. On the other hand, when the interval between two note points is over 40 seconds, this similarity notably decreases to 0.39. This suggests that the density of overlapping information significantly influences the degree of resemblance between expanded notes.
We noticed that when two points are taken less than 10 seconds apart, they tend to exhibit a high degree of similarity, with an average score \cite{sbert, ethayarajh2019contextual, gao2019representation} of 0.63. This could be because they share a lot of overlapping information. If note points are more than 40 seconds apart, their similarity drops to 0.39, showing that less overlap means less similarity.

\subsubsection{Error in LLM generation.} \texttt{GPT-4} sometimes fails to generate the requested note. For example, P7 wrote a micronote to note down her thoughts that are not directly discussed in the video. The model replied with - \textit{`Please provide the transcript related to the keypoint so I can assist you in creating a note.'}. The occurrence of such error is 0.72\% (4 out of 559 total calls). 
